The motion of chondrules and other particles in a protoplanetary disc with temperature fluctuations

We consider the mechanism of photophoretic transport in protoplanetary disks that are optically thick to radiation. Here, photophoresis is not caused by the central star but by temperature fluctuations that subject suspended solid particles, including chondrules, to non-isotropic thermal radiation within the disk. These short-lived temperature fluctuations can explain time-of-flight size sorting and general number density enhancements. The same mechanism will also lead to velocity fluctuations of dust aggregates beyond $100\,\mathrm{m\,s^{-1}}$ for mm-sized particles in protoplanetary disks. Applying this in future research will change our understanding of the early phases of collisional dust evolution and aggregate growth as particles cross the bouncing barrier and as mass transfer rates are altered.

==> fluctuations_sketch.tex <==
\begin{tikzpicture}[
interface/.style={
	% The border decoration is a path replacing decorator. 
	% For the interface style we want to draw the original path.
	% The postaction option is therefore used to ensure that the
	% border decoration is drawn *after* the original path.
	postaction={draw,decorate,decoration={border,angle=-45,
			amplitude=0.5cm,segment length=4mm}}},
]

\def\X{-5.5} % Wand-Position
\def\L{10} % Wand-Höhe
\def\O{7} % Verschiebung Kugel-Würfel
\def\R{1.5} % sphere radius
\def\angEl{30} % elevation angle
\def\angAz{-115} % azimuth angle
\tikzset{xyplane/.style={cm={cos(\angAz), sin(\angAz)*sin(\angEl), -sin(\angAz), cos(\angAz)*sin(\angEl), (0,-1.2*\R)}}}

% Walls
\fill[white,fill=lightgray,opacity=0.2,rounded corners] (\X-0.5,1.5*\R) rectangle (\X,-\L);
\draw[darkgray,line width=.5pt,interface](\X,1.45*\R)--(\X,-\L+0.1) node[left=0.5em,above=1em,pos=0] {Wall A};
\draw[darkgray,line width=.5pt,interface](-\R,2.5*\R-\O)--(-\R,1.05*\R-\O) node[right=2.5em,above=0em,pos=0.5] {Wall B};
%\draw[darkgray,line width=.5pt,interface](0.5*\R,2.5*\R-\O)--(0.5*\R,1.05*\R-\O);
%% vertical dashed line
%\draw[dashed,gray](0,-1.5)--(0,\M);
%% coordinates system
%%\draw(0,0.15)node[above]{$x$};
%%\draw[<->,line width=1pt] (1,0) node[above]{$y$}-|(0,-1) node[left]{$z$};

% Kugel
\filldraw[shading=ball, ball color=white, draw=lightgray] (0,0) circle (\R);
%%\fill[shading=ball, ball color=white] (0,0) circle (\R);
%\foreach \t in {-80,-50,-25,0,25,50,80} { \DrawLatitudeCircle[\R,gray]{\t} } %; \draw[current plane,dashed,red] (\angVis:1) arc (\angVis:180-\angVis:1); }
%\foreach \t in {15, 60, 105, 150} { \DrawLongitudeCircle[\R,gray]{\t} }
%\begin{scope}[
%rotate around={0:(0,0)},
%decoration={
%	markings,
%	mark=at position 0.45 with {\arrow{>}},
%	mark=at position 0.79 with {\arrow{>}},
%	%mark=at position 0.9 with {\arrow{>}}
%}
%]
%\DrawLongitudeCircle[\R,gray]{130}
%\draw[current plane, white, very thick, postaction={decorate}] (90:1) arc (90:180+\angVis:1) node[pos=0.43, right=0.3ex] {$\boldsymbol{T\left(\zeta\right)}$};
%\draw[current plane,white,very thick,dashed] (180+\angVis:1) arc (180+\angVis:270:1);
%\end{scope}

% Würfel
\filldraw[lower left=darkgray!60,lower right=lightgray, upper left=lightgray!20,upper right=darkgray!60, draw=darkgray!20, thick] (-\R,-\R-\O) rectangle (\R,\R-\O);

% charakteristische Punkte
\pgfmathsetmacro\xa{-1.1*\R*cos(30)}
\pgfmathsetmacro\xb{-1.1*\R*cos(0)}
\pgfmathsetmacro\ya{1.1*\R*sin(30)}
\pgfmathsetmacro\xc{-1.1*\R*cos(10)}
\pgfmathsetmacro\yc{-1.1*\R*sin(10)}
\pgfmathsetmacro\xd{-1.1*\R*cos(60)}
\pgfmathsetmacro\yd{-1.1*\R*sin(60)}
\pgfmathsetmacro\xe{-1.1*\R*cos(110)}
\pgfmathsetmacro\ye{-1.1*\R*sin(110)}
%\coordinate[mark coordinate] (O) at (0,0);% node[right] {$O$};
%\coordinate[mark coordinate] (N) at (0,\H);
%\coordinate[mark coordinate] (S) at (0,-\H);

%% setze Buchstabend und zeichen Linien
%\path (N) +(-0.6ex,-0.8ex) node[left] {$\zeta=0$};
%\path (S) +(-0.6ex,0.8ex) node[left] {$\zeta=\pi$};
%%\draw[thin,<->] (-0.06*\R,0) -- (-0.06*\R,\H);
%%\node[left,rotate=90] at (-0.15*\R,1/2*\H) {$\mathbf{r_0}$};
%\draw[thin,blueThesis,decorate,decoration={brace,raise=0.5pt,amplitude=1ex}] (N) -- (O)
%node[midway,right=1ex] {$\boldsymbol{r_0}$};

%% Koordinaten-Achsen
%\draw[thick,->] (0,\H) -- (0,1.4*\R) node[above] {$z$};
%\draw[thick,dashed,-] (0,-\R) -- (0,\H);
%\draw[thick,-] (0,-1.1*\R) -- (0,-\R);
%%\draw[xyplane,thick,<->] (1.8*\R,0) node[below] {$x$} -- (0,0) -- (0,2.0*\R)    node[right] {$y$};

\def\RadA{-3.5*\R}
\def\RadB{-2.5*\R}
\def\RadC{-6*\R}

% Strahlung
\begin{scope}[
	decoration={markings,mark=at position 0.5 with \arrow{>}},
	orangeThesis,
	thick
	%very thick
	]

\draw[postaction=decorate] (\X,0) -- (\xa,\ya);% node[above=3em,pos=0.5, align=left] {radiative flux\\$\boldsymbol{I\propto\sigma_\textbf{SB}T^4}$};
\draw[postaction=decorate] (\X,0) -- (\xb,0);
\draw[postaction=decorate] (\X,0) -- (\xa,-\ya);

\draw[postaction=decorate] (\X,\RadA) -- (\xc,\yc);
\draw[postaction=decorate] (\X,\RadA) -- (\xd,\yd);
\draw[postaction=decorate] (\X,\RadA) -- (\xe,\ye);

\draw[postaction=decorate] (\X,\RadB) -- (-1.1*\R,-\O+0.9*\R);
\draw[postaction=decorate] (\X,\RadB) -- (-1.1*\R,-\O+0.5*\R);
\draw[postaction=decorate] (\X,\RadB) -- (-1.1*\R,-\O+0.1*\R);
\draw[postaction=decorate] (\X,\RadB) -- (-1.1*\R,-\O-0.3*\R);
\draw[postaction=decorate] (\X,\RadB) -- (-1.1*\R,-\O-0.7*\R);

\draw[postaction=decorate] (\X,\RadC) -- (-1.1*\R,-\O+0.8*\R);
\draw[postaction=decorate] (\X,\RadC) -- (-1.1*\R,-\O+0.4*\R);
\draw[postaction=decorate] (\X,\RadC) -- (-1.1*\R,-\O+0.0*\R);
\draw[postaction=decorate] (\X,\RadC) -- (-1.1*\R,-\O-0.4*\R);
\draw[postaction=decorate] (\X,\RadC) -- (-1.1*\R,-\O-0.8*\R);
\end{scope}


\end{tikzpicture}
